Distributed Rate Adaptation and Power Control in Fading Multiple Access Channels

Traditionally, the capacity region of a coherent fading multiple access channel (MAC) is analyzed in two popular contexts. In the first, a centralized system with full channel state information at the transmitters (CSIT) is assumed, and the communication parameters like transmit power and data-rate are jointly chosen for every fading vector realization. On the other hand, in fast-fading links with distributed CSIT, the lack of full CSI is compensated by performing ergodic averaging over sufficiently many channel realizations. Notice that the distributed CSI may necessitate decentralized power-control for optimal data-transfer. Apart from these two models, the case of slow-fading links and distributed CSIT, though relevant to many systems, has received much less attention. In this paper, a block-fading AWGN MAC with full CSI at the receiver and distributed CSI at the transmitters is considered. The links undergo independent fading, but otherwise have arbitrary fading distributions. The channel statistics and respective long-term average transmit powers are known to all parties. We first consider the case where each encoder has knowledge only of its own link quality, and not of others. For this model, we compute the adaptive capacity region, i.e. the collection of average rate-tuples under block-wise coding/decoding such that the rate-tuple for every fading realization is inside the instantaneous MAC capacity region. The key step in our solution is an optimal rate allocation function for any given set of distributed power control laws at the transmitters. This also allows us to characterize the optimal power control for a wide class of fading models. Further extensions are also proposed to account for more general CSI availability at the transmitters.

==> proof_appB.tex <==
Let us first find an upper bound for the expected sum-rate of any achievable scheme.
\begin{align}
\sum_{i=1}^N E[R_i(H_i)] = 
        \sum_{i=1}^N\int_{0}^{\infty} & R_i(h_i) d\psi_i(h_i)
\end{align}
%Using Definition~\eqref{def:inv:cdf} (similar to the discrete case), %let $h_i(x)$ denote the inverse cdf  $\psi^{-1}_i(x)$. 
Using similar steps as in the discrete-state derivation in \eqref{eq:thpf3}, we get
by the sum-rate bound of the $N$ user MAC capacity region (see \cite{GamalKim11}),
\begin{align}
\sum_{i=1}^N E[R_i(H_i)] 
%       &=\int_0^1 R_1(h_1(x)) d(x)\, +\int_0^1 R_2(h_2(x)) dx \notag \\
%       &=\int\limits_0^1 (R_1(h_1(x))+ R_2(h_2(x))) dx  \notag \\
        \leq \int\limits_0^1 \frac 12 \log(1+\sum_{j=1}^{N}h_j^2(x)P_j)\,dx \notag,
\end{align}

thus obtaining an upper bound to the achievable sum-rate.

We will also show that this upper bound is in fact achieved by the rate-allocations
prescribed in Theorem~\ref{th:discretemult}. The rest of the
proof follows from Lemmas~\ref{lem:multwo} and \ref{lem:mulone} presented
below.

\begin{lemma} \label{lem:multwo}
For $x\in[0,1]$ and the rate allocation in \eqref{eq:adptcpmult},
$$
\sum_{i=1}^NR_i(h_i(x)) = \frac 12 \log(1+ \sum_{j=1}^Nh_j^2(x)P_j).
$$
\end{lemma}
\begin{IEEEproof}
From the rate allocation in  Theorem~\ref{th:discretemult}, it follows that
$$\sum_{i=1}^NR_i(h_i(0)) = \frac 12 \log(1+ \sum_{j=1}^Nh_j^2(0)P_j)$$
Also, for $x >0$, 
{\allowdisplaybreaks
\begin{align}
\sum_{i=1}^NR_i(h_i(x)) &=\sum_{i=1}^NR_i(h_i(0))+\sum_{i=1}^N \int_{0}^{x} \frac{h_i(y)P_id(h_i(y))}{1+\sum_{j=1}^{N}h_j(y)^2P_{j}} \notag \\
&=\frac 12 \log(1+ \sum_{j=1}^Nh_j^2(0)P_j)+\sum_{i=1}^N \int_{0}^{x} \frac{h_i(y)P_id(h_i(y))}{1+\sum_{j=1}^{N}h_j(y)^2P_{j}} \notag \\
 &=\frac 12 \log(1+ \sum_{j=1}^Nh_j^2(0)P_j)+\int\limits_{0}^{x} \frac{\sum_{k=1}^{N}h_k(y)P_{k}d(h_k(y))}{1+\sum_{j=1}^{N}h_j(y)^2P_{j}} \notag \\
        &=\frac 12 \log(1+ \sum_{j=1}^Nh_j^2(0)P_j)+\int\limits_{1+ \sum_{j=1}^Nh_j^2(0)P_j}^{1+\sum_{k=1}^{N}h_k^2(x)P_k} \dfrac{1}{2p}\,dp \\
        &=\dfrac{1}{2}\log(1+\sum_{k=1}^{N}h_k^2(x)P_k).
\end{align}
}
This completes the proof of the lemma.
\end{IEEEproof}


\begin{lemma} \label{lem:mulone}
The rate allocation given in \eqref{eq:adptcpmult} is outage-free.
\end{lemma}
\begin{IEEEproof}
We will show that $\forall (h_1(x_1),h_2(x_2),\cdots h_N(x_N)) \in \bar H$ such that $0 \leq x_i \leq 1$, $1 \leq i \leq N$  and $ \forall S \subseteq \{1,2,\cdots,N\}$
\begin{align*}
 \sum_{i \in S}R_i(h_i(x_i))  &\leq \frac 12 \log(1+\sum_{i\in S} h_i(x_i)^2 P_i ).
\end{align*}


Let $|S|$ denote the cardinality of the set $S$ and
 let $L$ be the vector formed by reading from left to right the indices of $x_i,~i \in S$ arranged in increasing order.
Let $L(l)$ denote the value of the $l^{th}$ component of $L$. Hence,  $x_{L(1)} \leq x_{L(2)} \leq \cdots \leq x_{L_{|S|}}$.

{\allowdisplaybreaks
\begin{align}
 \sum_{i\in S}R_i(h_i) &=\sum_{i \in S}R_i(h_i(0))+\sum_{i\in S} \int_{0}^{x_i} \frac{h_i(y)P_id(h_i(y))}{1+\sum_{j=1}^{N}h_j(y)^2P_{j}} \notag \\
& \leq \frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{i=1}^{|S|} \int_{0}^{x_{L(i)}} \frac{h_{L(i)}(y)P_{L(i)}d(h_{L(i)}(y))}{1+\sum_{j=1}^{N}h_j(y)^2P_{j}}\notag\\
&\leq \frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{i=1}^{|S|} \int_{0}^{x_{L(i)}} \frac{h_{L(i)}(y)P_{L(i)}d(h_{L(i)}(y))}{1+\sum_{j=1}^{|S|}h_{L(j)}(y)^2P_{j}}\label{musrone} \\
&=\frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{k=1}^{|S|} \sum_{i=k}^{|S|}\int_{x_{L(k-1)}}^{x_{L(k)}} \frac{h_{L(i)}(y)P_{L(i)}d(h_{L(i)}(y))}{1+\sum_{j=1}^{|S|}h_{L(j)}(y)^2P_{j}} \notag \\
&=\frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{k=1}^{|S|}\int_{x_{L(k-1)}}^{x_{L(k)}}\frac{\sum_{i=k}^{|S|}h_{L(i)}(y)P_{L(i)}d(h_{L(i)}(y))}{1+\sum_{j=1}^{|S|}h_{L(j)}(y)^2P_{j}} \label{ust2}
\end{align}
}

where $x_{L(0)}:=0$. Also, we have $x_{L(j)} \leq x_{L(k-1)} \leq x_{L(k)}$ for $j \leq k-1$.

\begin{align}
 \sum_{i\in S}R_i(h_i) & \leq \frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{k=1}^{|S|}\int_{x_{L(k-1)}}^{x_{L(k)}}\frac{\sum_{i=k}^{|S|}h_{L(i)}(y)P_{L(i)}d(h_{L(i)}(y))}{1+\sum_{j=1}^{k-1}h_{L(j)}^2(x_{L(j)})P_{L(j)}+\sum_{j=k}^{|S|}h_{L(j)}^2(y)P_{L(j)}} \notag \\
&=\frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\sum_{k=1}^{|S|}\int_{1+\sum_{j=1}^{k-1}h_{L(j)}^2(x_{L(j)})P_{L(j)}+\sum_{j=k}^{|S|}h_{L(j)}^2(x_{L(k-1)})P_{L(j)}}^{1+\sum_{j=1}^{k-1}h_{L(j)}^2(x_{L(j)})P_{L(j)}+\sum_{j=k}^{|S|}h_{L(j)}^2(x_{L(k)})P_{L(j)}}\frac{dp}{2p} \label{ust3} 
\end{align}

where the empty summation is defined to be 0, i.e. $\sum_{j=1}^0 h_{L(j)}^2(x_{L(j)})P_{L(j)}=0$.

Simplifying equation \eqref{ust3},
\begin{align}
 \sum_{i\in S}R_i(h_i) &\leq \frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i )+\frac 12 \log(1+\sum_{i=1}^{|S|}h_{L(i)}^2(x_{L(i)})P_{L(i)})-\frac 12 \log(1+\sum_{i\in S} h_i^2(0) P_i ) \notag\\
&=\frac 12 \log(1+\sum_{i\in S}h_i^2(x_i)P_i)\notag
\end{align}

This proves the claim.


\end{IEEEproof}


